Why Train More? Effective and Efficient Membership Inference via Memorization

Membership Inference Attacks (MIAs) aim to identify specific data samples within the private training dataset of machine learning models, leading to serious privacy violations and other sophisticated threats. Many practical black-box MIAs require query access to the data distribution (the same distribution where the private data is drawn) to train shadow models. By doing so, the adversary obtains models trained "with" or "without" samples drawn from the distribution, and analyzes the characteristics of the samples under consideration. The adversary is often required to train more than hundreds of shadow models to extract the signals needed for MIAs; this becomes the computational overhead of MIAs. In this paper, we propose that by strategically choosing the samples, MI adversaries can maximize their attack success while minimizing the number of shadow models. First, our motivational experiments suggest memorization as the key property explaining disparate sample vulnerability to MIAs. We formalize this through a theoretical bound that connects MI advantage with memorization. Second, we show sample complexity bounds that connect the number of shadow models needed for MIAs with memorization. Lastly, we confirm our theoretical arguments with comprehensive experiments; by utilizing samples with high memorization scores, the adversary can (a) significantly improve its efficacy regardless of the MIA used, and (b) reduce the number of shadow models by nearly two orders of magnitude compared to state-of-the-art approaches.

==> sec_contents/2_background.tex <==
\section{Background}
\label{sec:background}

%\varun{mostly notation and formalisms; maybe good place to introduce the membership inference game}
In this section, we introduce the background and formalism that we use through the paper. 

\subsection{Machine Learning}
\label{subsec:ml}

\noindent{\bf 1. Supervised Machine Learning:} Let us assume the existence of a distribution $P$ that captures the space of inputs and outputs, from which a dataset $D$ of size $t$ is sampled (\ie $D \sim P^n$) such that $D = \{z_i\}_{i=1}^n$. Each $z$ is of the form $(x,y)$, where $x \in \mathcal{X}$ is the space of inputs and $y \in \mathcal{Y}$ is the space of outputs; for example, $\mathcal{X}$ can be thought of as the space of images, and $\mathcal{Y}$ can be thought of as labels for the images, as in the CIFAR-10 dataset~\cite{krizhevsky2010convolutional}. Using this dataset, a learning algorithm $L$ (\eg stochastic gradient descent~\cite{bottou2012stochastic}) can create a trained model \ie $h \sim L(D)$ by minimizing a suitable objective $\mathcal{L}$ (\eg cross-entropy loss~\cite{zhang2018generalized}). 

%\vspace{2mm}
\noindent{\bf 2. Membership Inference Attacks (MIAs):} For many applications, ML models are trained on large corpora of data, some of which is sensitive and private~\cite{shokri2017membership}. Membership inference is a class of attacks on the privacy of the data used to train the model, and are training distribution-aware~\cite{yeom2018privacy,shokri2017membership,carlini2022membership,jayaraman2020revisiting,song2021systematic,murakonda2021quantifying,ye2021enhanced,sablayrolles2019white}. In particular, adversaries aim to infer if a particular sample (or group of samples) was present in the training dataset given access to a trained model. They often do so by checking for effects due to the presence or absence of the point under consideration on a large set of shadow models -- those that are trained on varying data subsets to estimate these effects. MIAs were used to test if data is successfully deleted from ML models~\cite{bourtoule2021machine}, with some caveats~\cite{kong2023can}. Additionally, data deletion is also susceptible to MIAs~\cite{chen2021machine}. Carlini \etal~\cite{carlini2022membership} argue that the efficacy of attacks should be measured through the ability to successfully identify members (true positive rate) at low false positive rate regimes, as commonly done in other areas of computer security.

%\varun{add some implications of MI and how this is not good for privacy and how it's been used in data deletion settings for verification too}
%\shruti{Emphasize that for adversarial setting, precision of the attack is important i.e., high TP at low FP, and hence important to identify the most vulnerable points. }

%\vspace{2mm}
\noindent{\bf 3. Membership Inference Game:} The game below defines what the objective of the MI adversary is. The game defines the interaction between two parties: an adversary aiming to perform MI, and a challenger that is responsible for training. We assume a strong model where the adversary controls all but one point, as done by Mahloujifar \etal~\cite{mahloujifar2022optimal}.
%\varun{add a reference to saeed's paper + a note that we consider a strong adversary that controls the dataset + add a reference to yeom's paper for the advantage definition}  \shruti{The above section talks about inferring a particular point but the below game is for detecting a set of points. May be adding the range for '$n$' will help. Do we consider '$n=1$'}
\begin{enumerate}
\itemsep0em 
\item An adversary picks a dataset $D=\{z_1,\cdots,z_n\}$ and datapoints $D_{adv} = \{z'_j\}_{t=1}^t$ (for $t \geq 1$). 
\item A challenger samples a bit $b$ uniformly at random and creates
\[
  D' = \left.
  \begin{cases}
    D \cup D_{adv} & \text{if } b=1 \\
    D & \text{if } b=0 \\
  \end{cases}
  \right\}
\]
\item The challenger learns a model $h$ by running $L(D')$ and sends $h$ to the adversary.
\item The adversary guesses a bit $b'$, and wins if $b' = b$.
\end{enumerate}

The advantage with which such an adversary (represented as algorithm $\calA$ which returns an output $\{0,1\}$) is defined as the difference between $\calA$’s true and false positive rates~\cite{yeom2018privacy}. Formally,
\begin{equation}
\label{eq:advantage}
\adv = \Pr[b'=0 | b=0] - \Pr[b'=0 | b=1]
\end{equation}


\noindent{\bf 4. Stability \& Memorization:} ML models are vastly overparameterized, and are known to fit to even random labels~\cite{feldman2020longtail}. This is termed memorization. For a sample $z_i$, given dataset $D$ (without $z_i$), label memorization is formalized as follows:
\begin{equation}
\label{eq:memorization}
\text{mem}(L,D,z_i) := \mathop{Pr}_{h \sim L(D^{(i)})}[h(x_i) = y_i] - \mathop{Pr}_{h \sim L(D)}[h(x_i) = y_i]   
\end{equation}
where $D^(i) = D \cup \{z_i\}$. We term the value of Equation~\ref{eq:memorization} as a memorization score.

\noindent {\em Stability} aims to understand how much the output of learning algorithms changes with minor perturbations to the input~\cite{koh2017understanding}. A stable learning algorithm is one where the output does not change with changes in inputs. We define Leave-One-Out (LOO) stability as done by Feldman~\cite{feldman2020longtail}:
\begin{gather*}
\label{eq:loostab}
    \text{LOOStab}(P, L) = 
    \frac{1}{n}\sum_{i=1}^n \mathop{\mathbb{E}}_{D \sim P^n}\left[|\text{mem}(L,D,z_i)|\right]
    %\frac{1}{n}\sum_{i=1}^n \mathop{\mathbb{E}}_{D \sim P^n}\left[|\mathop{Pr}_{h \sim L(D^{(i)})}[h(x_i)=y_i] - \mathop{Pr}_{h \sim L(D)}[h(x_i)=y_i]|\right]
\end{gather*}
This results in the following lower bound:
\begin{equation}
\label{eq:loostab-mem}
    \frac{1}{n} \mathop{\mathbb{E}}_{D \sim P^n}\left[\sum_{i=1}^n\text{mem}(L,D,z_i)\right] \leq     \text{LOOStab}(P, L)
\end{equation}

%\vspace
% \noindent{\bf Note 1:} Feldman~\cite{feldman2020longtail} notes that the aforementioned definition of memorization is measuring the TV distance between distributions of the indicator of the label being $y_i$.

%\vspace
% \noindent{\bf Note 2:} Here $P$ can be used interchangeably with $P$. We avoid doing so to enable ease of understanding.

% \subsection{Out-of-distribution Detection}


%We can partition the potential worlds of the membership inference game into two categories (\jihye{cite Shokri's recent paper}): given a single challenge point $z'$,
% We sample $m$ observations from \textbf{in} world (or \textbf{out} world), which are characterized by distribution $P$ (or $Q$).
% %Let $P$ be the distribution of signal function outputs in \textbf{in} world, and $Q$ be the distribution corresponding to \textbf{out} world. 
% For instance, in Carlini's attack, an observation correspond to the scaled logit value from a shadow model trained with a random subset of entire traing dataset.

%   \varun{add more text for memorization}

\subsection{Hypothesis Testing}
\label{subsec:hypo_testing}
\jihye{let us be more formal in viewing MI Game from hypothesis testing view point. I'll make separate file for sec2 and bring some from Somesh's note}
\jihye{let us be more formal in viewing MI Game from hypothesis testing view point. I'll make separate file for sec2 and bring some from Somesh's note}
%\varun{to do: add some blurb on hypothesis testing and change the notation to P and Q}
A hypothesis test is a method of statistical inference where one uses the data at hand is sufficient to support a particular hypothesis. As an example, a hypothesis test can be used to determine if samples of data are sourced from distribution $P$ or distribution $Q$, given access to observations $\mathcal{O} = \{o_1, \cdots, o_m\}$.

%\vspace{1mm}
\mypara{1. Log-Likelihood Ratio (LLR) Test:} There are two types of errors associated with hypothesis testing: 
\begin{itemize}
\itemsep0em
\item Type I: probability that the test outputs $Q$ if $P$ is true.
\item Type II: probability that the test outputs $P$ if $Q$ is true.
\end{itemize}
The ideal goal of a hypothesis test is to achieve Type I error below an application specific threshold. The Neyman-Pearson lemma~\cite{shaffer1995multiple} states that the LLR test achieves the best Type II error for a given bound on the Type I error (\ie the LLR test is optimal). That is, the LLR test outputs $P$ if
\begin{equation}
    \text{LLR}(O) = \frac{P(o_1, o_2, ..., o_m)}{Q(o_1, o_2, ..., o_m)} = \prod_{i=1}^m \frac{P(o_i)}{Q(o_i)} \geq 1
\end{equation}
and otherwise outputs $Q$. 
% \varun{@jihye -- please check if the definitions are correct? i have a feeling i swapped the P and Q for the LLR test}

%Neyman-Pearson Lemma says that the exact optimal test for distinguishing $Q$ from $P$ is the LLR test defined above.

%\varun{maybe homogeneize the domain across definitions?}
%\vspace{1mm}
\noindent{\bf 2. Hellinger Distance:} For two distributions $P$ and $Q$ over some domain $\mathcal{X}$, the Hellinger distance between $P$ and $Q$ is given by
\begin{equation*}
    H(P, Q) = \frac{1}{\sqrt{2}} ||\sqrt{P} - \sqrt{Q}||_2
\end{equation*}
\begin{equation}
    H^2(P, Q) = \frac{1}{2} \int_\mathcal{X} ( \sqrt{P} - \sqrt{Q}) ^2 dx
\end{equation}

%\vspace{1mm}
\noindent{\bf 3. TV Distance:} %Consider a measurable space $(\Omega, \mathcal{F})$ and probability measures  $P,Q$ defined on $(\Omega, \mathcal{F})$. 
The total variation distance between  $P$ and $Q$ is
\begin{equation}
    \delta(P, Q) = \sup_{A}|P(A) - Q(A)|
\end{equation}
where $A$ is any measurable subset of the sampling space. 


\noindent{\em Note:} $H^2(P,Q) \leq \delta(P,Q) \leq \sqrt{2}H(P,Q)$

%\varun{use jihye's cmu note for notation definition here. what is the cmu note?}

==> sec_contents/5_theory.tex <==
\section{Connecting MI and Memorization}
\label{sec:theory}

Having provided some preliminary evidence that highlights the connections between label memorization and MI susceptibility, we wish to formalize the connection. In this section, we will first demonstrate that memorization is a lower bound for the MI advantage. Next, based on the previously discussed connection between MIA and hypothesis testing (refer \S~\ref{subsec:hypo_testing}), we proceed to show how memorization can reduce the computational burden associated with attackers with a lower bound for the number of samples need for distinguishing two distributions.

\vspace{1mm}
\mypara{Step 1. Connecting MI Advantage and Memorization:} By linearity of expectation, $\text{LOOStab}(P, L)$ can be denoted as
\begin{equation*}
\label{eq:can_1}
\mathop{\mathbb{E}}_{D \sim P^n}\left[\frac{1}{n}\sum_{i=1}^n |\mathop{Pr}_{h \sim L(D^{(i)})}[h(x_i)=y_i] - \mathop{Pr}_{h \sim L(D)}[h(x_i)=y_i]|\right]
\end{equation*}
and consequently,
\begin{equation*}
\label{eq:can_2}
\adv \geq \text{LOOStab}(P, L)
\end{equation*}
and by definition,
\begin{equation*}
\label{eq:final}
\adv \geq \frac{1}{n} \mathop{\mathbb{E}}_{D \sim P^n}\left[\sum_{i=1}^n\text{mem}(L,D,z_i)\right] 
\end{equation*}

When $n=1$ and for a fixed point $z$, we can see that:

\begin{tcolorbox}
\begin{equation}
\label{eq:final_single}
\texttt{Adv}(\mathcal{A}, L, 1, P) \geq \text{mem}(L,\{z\},z) 
\end{equation}
\end{tcolorbox}

\noindent{\bf Implications:} \varun{populate? caveat: how do we get mem score? we assume an oracle gives it to us -- future work will tackle making this process tractable}

Before we proceed to the next step, recall that Ye \etal~\cite{ye2021enhanced} formalize MIA in the hypothesis testing framework. For a point $z'$ chosen by the adversary, they define two worlds:
\begin{enumerate}
\itemsep0em
\item The \textbf{in} world, where $z'$ is a member of the training data $D'$, characterized by distribution $\Pin$. 
\item The \textbf{out} world, where $z'$ is a non-member of training data $D'$, characterized by distribution $\Pout$. 
\end{enumerate}
Given $z'$ and a set of observations $o$ (\eg predictions of models, or shadow models trained on differing subsets of data etc.), the goal of an MIA is to determine whether $o$ was drawn from $\Pin$ or $\Pout$. This can be viewed as the standard hypothesis testing setting as follows:
%\vspace{1mm}
% \begin{center}
% \fbox{
% \begin{minipage}{21em}
%\noindent 
given two known distributions $\Pin$ and $\Pout$ over a domain $\mathcal{O}$ and a set of $m$ i.i.d. observations $\hat{O} = \{o_1, o_2, . . . , o_m\}$ generated from an unknown distribution $R \in {\Pin, \Pout}$, a simple hypothesis test asks which of the following two hypotheses is true: 1. $H_0 : R = \Pin$, or 2. $H_1 : R = \Pout$.
% \end{minipage}
% }
% \end{center}

\vspace{1mm}
\mypara{Step 2. Connecting MI Advantage and Hellinger Distance:} The advantage of a hypothesis test $T$ for a set of observations $\hat{O} =\{o_1, o_2, ..., o_m\}$ is
\begin{equation*}
    \texttt{Adv}(T, m, (\Pin, \Pout)) = \pr_{\hat{O} \sim \Pin}[T(\hat{O}) = \Pin] - \pr_{\hat{O} \sim \Pout}[T(\hat{O}) = \Pin]
\end{equation*}
This is semantically identical to the advantage of an MI adversary as defined earlier. From Theorem 2.1 in Cannone \etal~\cite{canonne2019structure}, when $T$ specifically becomes soft LLR (sLLR) test as 
\begin{equation*}
\label{eq:adv_sllr}
    \text{sLLR}(\hat{O}) = \Pin ~\text{w.p. proportional to $\exp(\frac{\text{LLR}(\hat{O})}{2})$}
\end{equation*}
Using the above information, for $m=1$, we can restate the advantage as
\begin{equation*}
\label{eq:adv_adv_llr_1}
    {\texttt{Adv} (\text{sLLR}, 1, (\Pin, \Pout))} = H^2(\Pin,\Pout)
\end{equation*}
%\end{tcolorbox}
Thus, for the best hypothesis test $T^*$ (\ie LLR test),
\begin{tcolorbox}
\begin{equation}
\label{eq:adv_llr_1}
{\texttt{Adv} (T^*, 1, (\Pin, \Pout))} \geq H^2(\Pin,\Pout)
\end{equation}
\end{tcolorbox}

For $m>1$, we have
%\begin{tcolorbox}
\begin{equation}
\label{eq:adv_llr_m}
    \advhyp \geq 1 - \exp(-m \frac{H^2(\Pin, \Pout)}{2})
\end{equation}
%\end{tcolorbox}
(abusing some constants)

\vspace{2mm}
From equations~\ref{eq:final_single} and~\ref{eq:adv_llr_1}, we can see that there exists some constant $k_z$ s.t.
\begin{equation}
\label{eq:connection}
    H^2(\Pin,\Pout) = k_z \cdot \text{mem}(L,\{z\},z)
\end{equation}

\varun{change this based on the bound with TV distance}

\mypara{STEP 3: Connecting Sample Complexity and Memorization}


\begin{itemize}
\itemsep0em
\item For a test $T$ and distributions $P$ and $\Pout$, let $m_\delta^T(\Pin,\Pout)$ be the sample complexity of $T$ such that for every $m \geq m_\delta^T(\Pin,\Pout)$ the advantage is $\frac{2}{3}$. 
\item Let $m_\delta^*(\Pin,\Pout)$ be the sample complexity of optimal hypothesis test.
% be the minimum number
% of samples necessary to achieve an error probability $\delta$.
\end{itemize}

The sample complexity of the optimal hypothesis test between $\Pin$ and $\Pout$ is
\begin{equation}
\label{eq: optimum-sample}
    m_\delta^*(\Pin,\Pout) = \Theta (\frac{1}{H^2(\Pin, \Pout)})
\end{equation}
(by setting $m = \Theta (\frac{1}{H^2(\Pin, \Pout)})$ in eqn.~\ref{eq:adv_llr_m}, the advantage is at least $\frac{2}{3}$).

\vspace{3mm}

\varun{expand this implication bit below; first introduce some notion of how MIAs are performed using shadow models + then explain how this number can be calibrated based on bound below}
Put another way, if one is to determine if sample $z$ comes from distribution $\Pin$ or not, the number of shadow models one needs to train (for performing an MI attack, based on equation~\ref{eq:connection}) is 

\begin{tcolorbox}
\begin{equation}
\label{eq: optimum-sample}
    m_\delta^*(\Pin,\Pout) = \Tilde{\Theta}(\frac{1}{\text{mem}(L,\{z\},z)})
\end{equation}
\end{tcolorbox}

%which is the sample complexity of LLR test, and in turn, the optimal sample complexity for distinguishing $\Pout$ from $P$.


